A Software Ecosystem Reshaped by a Paradigm Shift: the CSI-Piemonte Case

Context: Changes in the software development paradigm, when operated by entities with a pivotal role, have the power to affect a number of groups and entities in their sphere of influence, changing both their working habits and relations. Objective: In this paper we present the organizational changes occurred in a software ecosystem as consequence of a technological change. In particular we examine the evolution of an MDD solution and the changing roles of the company promoting it, the public administrations and the sub-contractors. Method: The paper focuses on a single case study that encompasses the six years long evolution of a Model-driven development solution, starting from its conception until is recent open-source release, across five distinct phases. The history was analyzed jointly by software engineering academics and industrial managers directly involved in the case study. Results: A report of the ecosystem evolution from an idiographic perspective is reported. An analysis of the history allowed an abstraction that led to the identification of several distinct ecosystem evolution motifs. Conclusion: The motifs represent a set of key process areas for the evolution of a software ecosystem. They are potentially generalizable to other similar ecosystems. As such, they can be used by researchers to evaluate existing in-progress case studies, and by practitioners as a set of guidelines.

==> results.tex <==
\subsection{Phase 0}

At this stage the tool was freely adopted by developers willing to do that. A large portion of them decide to adopt the "advanced modality", i.e., they did not just generate an initial skeleton but they built a model of the service they were working on to have the possibility to later refine the model and use it during the whole life of the project.

There are no data about an improvement in productivity but the developers reported the impression of benefiting from adopting MDD.  Adoption at this stage was only driven by immediate productivity gains.

Nevertheless developers did not like to give up the full control on the code but still they felt the trade-off was worth while because in return they were shielded from some technical details about more difficult and less creative aspects, e.g. securitization.

The emerging success of the initial version of the tools made evident the need for integrating the tool within the an IDE and start thinking about a more organic solution.

\subsection{Phase 1}

The adoption of the MDD approach became larger but still limited to services and in particular to orchestrated services. The previous version of the tool \emph{csiskelgen} was substituted by the second \emph{servicegen}.

In this phase more confidence was gained about the maturity of the enabling technologies.



\subsection{Phase 2}

In this phase an analysis of the results of the pilot projects was conducted supporting with concrete data further decisions.

\FED{They should be compared to results without MDD-Tools}

Results report that:
\begin{itemize}
\item all the projects were completed in time and reached the goal set,
\item the projects had good productivity, even better than the expectations. This is particularly good because there was not prior experience with the MDD tools,
\item 20 persons learnt how to use the MDD tools,
\item at the end of 2009 some teams were able to utilize MDD Tools without the direct involvement of the authors of the tools,
\item the reception from designers \FED{progettisti nel testo in italiano} was good.
\end{itemize}

The first pilot project (the \emph{Bandi} project) was circa 1600 functions points (f.p.) worth. The toolset was evolved in the context of this project. To complete the project it had to diverge from the pure use of the tools, overriding some of the generated code. This pragmatic approach was considered tolerable in this particular case because it was the first relevant project using a full MDD approach. Nevertheless this impure approach caused difficulties in the maintenance phase and newer versions of the MDD tools were not adopted, keeping using old versions. Considering the project bear a part of the effort for the development of MDD-Tools (which were useful in many other projects, of course) still some of the developers considered positive the impact on productivity of the MDD-Tools considering the benefit on that single project. Some other developers disagreed instead.

Other three pilot projects were developed:
\begin{itemize}
\item {\bf Turf}, \emph{Oct. 2009 - Feb. 2010, 1091 f.p.} - the overall productivity of the project was 32 f.p. per person-month (as a reference the typical productivity is 15 f.p. per p.m.) while the productivity of the bare development activities was 80 f.p./p.m. (the typical value is 30 f.p./p.m.), \FED{From where the 15 and the 30 come from? What is included in the development activities?}
\item {\bf Gerica}, \emph{Aug. 2009 - Dec. 2009, 345 f.p} -  the productivity of the bare development activities was 48 f.p./p.m. (the typical value is 30 f.p./p.m.),
\item {\bf Sicee}, \emph{14th Sept. 2009  - 27th Oct. 2009, 307 f.p.} - the overall productivity of the project was 39 f.p. per person-month (as a reference the typical productivity is 15 f.p. per p.m.) while the productivity of the bare development activities was 89 f.p./p.m. (the typical value is 30 f.p./p.m.).
\end{itemize}

In the case of {\bf Turf} project it was possible to develop two prototypes to support the customer in determining the requirements. The prototypes were developed in a short time thanks to the generation capabilities of the toolset and once the customer picked up one it could be evolved completing the missing logic. Without MDD tools the prototypes should have been both thrown away. Another advantage was the large flexibility guaranteed by this approach which permitted to face changes in requirements triggered by the customer.

The productivity of the {\bf Gerica} project was partially diminished by the particular form of the database.

The particularity of the {\bf Sicee} project was the tight schedule which permitted to verify the MDD approach under stress.

In general the results were considered positive and the organization gain the confidence for a larger adoption of the MDD Tools.

\subsection{Phase 3}

At this point the company did not see anymore the MDD approach as a risk. It was convinced by positive results on many different projects. 

Organizational issues had an effect on how the MDD tools are seen. The company decided to rely more and more on external suppliers, diminishing the percentage development produced internally therefore question arises about how the tools match this approach which was initially seen as well suited for internal development.

Finally the global crises affected also the possibility of performing new investments in the tool suite. While investments could not continue at the same pace as before it was clear that the users need to be supported.

In this period some developers started to act as evangelists in different business units.

There were minor resistances due to the fact that particular functionalities were difficult to develop with the tool suite but in general the trade off with the increased robustness, quality and efficiency of the development process were seen as satisfying.

\subsection{Phase 4}

At the time writing this phase is still in its early stages and results can not be properly documented.
